Pretraining with Artificial Language: Studying Transferable Knowledge in Language Models

We investigate what kind of structural knowledge learned in neural network encoders is transferable to processing natural language. We design artificial languages with structural properties that mimic natural language, pretrain encoders on the data, and see how much performance the encoder exhibits on downstream tasks in natural language. Our experimental results show that pretraining with an artificial language with a nesting dependency structure provides some knowledge transferable to natural language. A follow-up probing analysis indicates that its success in the transfer is related to the amount of encoded contextual information and what is transferred is the knowledge of position-aware context dependence of language. Our results provide insights into how neural network encoders process human languages and the source of cross-lingual transferability of recent multilingual language models.

==> sections/appendices/mlm-other-languages.tex <==
\section{Results from other languages}
\label{appendix:other-languages}

Here we present the result for \cref{sec:tilt-mlm} in Finnish and Japanese in \Figure{fig:tilt-mlm-results-fi} and \ref{fig:tilt-mlm-results-ja}.
The statistics of the dataset are show in \Table{tb:ud-statistics}.


\begin{table}[h]
  \centering
  \begin{tabular}{llrrr} \toprule
  Language & Dataset & \multicolumn{1}{c}{train} & \multicolumn{1}{c}{dev} & \multicolumn{1}{c}{test} \\ \midrule
  English  & EWT     & 16,688                     & 2,741                    & 2,911                     \\
  % Arabic   & NYUAD   & 12575                     & 1579                    & 1580                     \\
  Finnish  & FTB     & 11,502                     & 1,411                    & 1,482                     \\
  Japanese & BCCWJ   & 11,281                     & 2,218                    & 2,074                     \\
  % Korean   & Kaist   & 13956                     & 1226                    & 1366 \\
  \bottomrule
  \end{tabular}
  \caption{The number of sentences in the UD datasets used in the experiment.}
  \label{tb:ud-statistics}
\end{table}


\begin{figure*}[h]

\begin{minipage}{.60\linewidth}
\centering
\subfloat[The results of PoS tagging.]{\label{fig:tili-mlm-pos}\includegraphics[height=4.6cm]{data/tilt_mlm/pos_fi_frozen.png}}
\end{minipage}\hfill
\begin{minipage}{.40\linewidth}
\centering
\subfloat[The results of dependency parsing.]{\label{fig:tili-mlm-dep}\includegraphics[height=4.6cm]{data/tilt_mlm/dep_fi_frozen.png}}
\end{minipage}

\caption{The downstream performance on two syntactic tasks with the Finnish-FTB UD dataset.}
\label{fig:tilt-mlm-results-fi}
\end{figure*}

% \begin{tabular}{lcccccccccc}\toprule
%  & From scratch & Random weights & Uniform & Zipf & Random walk & Zipf Dep-flat & Zipf Dep-nested & English & Spanish & Japanese\\\midrule
%  PoS &  84.3±0.7   &    87.1±0.2    & 85.1±0.6 & 85.3±0.3 &   85.4±0.3  &    85.5±0.6   &     86.7±0.5    & 85.7±0.9 & 86.8±0.4 & 86.4±0.6\\
% Dep & 69.4±1.3   &    60.3±0.6    & 39.4±1.8 & 56.6±0.8 &   57.4±0.9  &    61.9±1.0   &     65.1±1.2    & 61.3±0.9 & 60.9±1.1 & 60.0±1.1\\
% \bottomrule
% \end{tabular}


\begin{figure*}[h]

\begin{minipage}{.60\linewidth}
\centering
\subfloat[The results of PoS tagging.]{\label{fig:tili-mlm-pos}\includegraphics[height=4.6cm]{data/tilt_mlm/pos_ja_frozen.png}}
\end{minipage}\hfill
\begin{minipage}{.40\linewidth}
\centering
\subfloat[The results of dependency parsing.]{\label{fig:tili-mlm-dep}\includegraphics[height=4.6cm]{data/tilt_mlm/dep_ja_frozen.png}}
\end{minipage}

\caption{The downstream performance on two syntactic tasks with the Japanese-BCCWJ UD dataset.}
\label{fig:tilt-mlm-results-ja}
\end{figure*}

% \begin{tabular}{lcccccccccc}\toprule
% & From scratch & Random weights & Uniform & Zipf & Random walk & Zipf Dep-flat & Zipf Dep-nested & English & Spanish & Japanese\\\midrule
%   PoS & 33.1±0.1   &    29.8±0.2    & 26.8±1.7 & 28.2±0.5 &   29.3±0.3  &    32.5±0.1   &     32.5±0.1    & 31.9±0.7 & 32.5±0.2 & 31.2±1.1 \\
 % & 33.2±0.0   &    32.6±0.0    & 13.8±7.3 & 32.4±0.2 &   32.2±0.3  &    31.9±0.4   &     32.8±0.2    & 32.0±0.8 & 32.4±0.4 & 32.3±0.4 \\
% \bottomrule
% \end{tabular}


Overall, we confirm that we observe similar trend as in English (\cref{sec:tilt-mlm}).
\PoSTagging{} does not seem to require structural knowledge, as indicated by less variance in the performance across pretraining languages.
In Finnish, the \RandomWeights{} baselines even outperforms the model trained from scratch ($84.3\pm0.7$ vs. $87.1\pm0.2$) in this hyper-parameter setting.
Pretraining with the unstructured languages provides lower scores than the \RandomWeights{} baseline overall, confirming the importance of structural knowledge encoded in the pretraining data.

We can also confirm that the \NestingDependency{} outperforms \FlatDependency{} in \DependencyParsing{} ($65.1\pm1.2$ vs. $61.9\pm1.0$ in Finnish, and $32.8\pm0.2$ vs. $31.9\pm0.4$ in Japanese).

Interestingly, in Finnish, the \NestingDependency{} language outperforms natural languages (\English{}, \Spanish{}, \Japanese{}), in contrast with the results from other languages where pretraining with natural languages performs better than \NestingDependency{} in English (\cref{sec:tilt-mlm-results}) and they exhibit comparable performance in the Japanese dataset (\Figure{fig:tilt-mlm-results-ja}).
We leave the investigation of this dataset or language-dependent difference to future work.

